Posterior accuracy and calibration under misspecification in Bayesian generalized linear models

Generalized linear models (GLMs) are popular for data-analysis in almost all quantitative sciences, but the choice of likelihood family and link function is often difficult. This motivates the search for likelihoods and links that minimize the impact of potential misspecification. We perform a large-scale simulation study on double-bounded and lower-bounded response data where we systematically vary both true and assumed likelihoods and links. In contrast to previous studies, we also study posterior calibration and uncertainty metrics in addition to point-estimate accuracy. Our results indicate that certain likelihoods and links can be remarkably robust to misspecification, performing almost on par with their respective true counterparts. Additionally, normal likelihood models with identity link (i.e., linear regression) often achieve calibration comparable to the more structurally faithful alternatives, at least in the studied scenarios. On the basis of our findings, we provide practical suggestions for robust likelihood and link choices in GLMs.

==> tables/descriptives-positive.tex <==
\begin{threeparttable}
\caption{Descriptive Statistics of Lower-bounded Results}
  \centering
    \begin{tabular}{|l|l||r|r|r|r|r|r|r|r|r|}
\hline
  \rule{0pt}{3ex} Link & Likelihood & DT & $P(\text{Conv.})$ & $\mathrm{RESS}_{\rm bulk}$ & $\mathrm{RESS}_{\rm tail}$ &  $\mr{TESS_{total}^{bulk}}$ \\
    \hline
    <%= paste_convergence(divergent_df, convergence_df[,3:ncol(convergence_df)], converged_models_df[,3:ncol(converged_models_df)], runtime_df[,3:ncol(runtime_df)], col_collapse= " & ", row_collapse="\\\\ \\hline ")%> \\
    \hline \hline
    \rule{0pt}{3ex} Link & Likelihood & PKs & $\mathrm{ELPD}_{\rm loo}$ & $\mathrm{bias}(\beta_{xy})$ & $\mathrm{SD}(\beta_{xy})$ & $\mathrm{RMSE}(\beta_{xy})$ \\
    \hline
    <%= paste_performance(pareto_k_df, predictive_metrics_df[,3:ncol(predictive_metrics_df)], recovery_metrics_df[,3:ncol(recovery_metrics_df)], col_collapse= " & ", row_collapse="\\\\ \\hline ")%> \\
    \hline
\end{tabular}%
     \begin{tablenotes}
      \tiny
      \item \textit{Note}: Most results are presented as mean(sd). $P(\text{Conv.})$ is calculated as a proportion of all models. $\mr{TESS_{total}^{bulk}}$ is also calculated using all models. Both the metrics for predictive performance and parameter recoverability are calculated only for models that had 10 or less divergent transitions and converged. In addition the parameter recoverability metrics are only shown for models using the true link. \\
    \end{tablenotes}
  \label{tab:positive-descriptives}%
\end{threeparttable}%


==> tables/descriptives-unit.tex <==
\begin{threeparttable}
\caption{Descriptive Statistics of Double-bounded Results}
  \centering
    \begin{tabular}{|l|l||r|r|r|r|r|r|r|r|r|}
\hline
  \rule{0pt}{3ex} Link & Likelihood & DT & $P(\text{Conv.})$ & $\mathrm{RESS}_{\rm bulk}$ & $\mathrm{RESS}_{\rm tail}$ &  $\mr{TESS_{total}^{bulk}}$ \\
    \hline
    <%= paste_convergence(divergent_df, convergence_df[,3:ncol(convergence_df)], converged_models_df[,3:ncol(converged_models_df)], runtime_df[,3:ncol(runtime_df)], col_collapse= " & ", row_collapse="\\\\ \\hline ")%> \\
    \hline \hline
    \rule{0pt}{3ex} Link & Likelihood & PKs & $\mathrm{ELPD}_{\rm loo}$ & $\mathrm{bias}(\beta_{xy})$ & $\mathrm{SD}(\beta_{xy})$ & $\mathrm{RMSE}(\beta_{xy})$ \\
    \hline
    <%= paste_performance(pareto_k_df, predictive_metrics_df[,3:ncol(predictive_metrics_df)], recovery_metrics_df[,3:ncol(recovery_metrics_df)], col_collapse= " & ", row_collapse="\\\\ \\hline ")%> \\
    \hline
\end{tabular}%
     \begin{tablenotes}
      \tiny
      \item \textit{Note}: Most results are presented as mean(sd). $P(\text{Conv.})$ is calculated as a proportion of all models. $\mr{TESS_{total}^{bulk}}$ is also calculated using all models. Both the metrics for predictive performance and parameter recoverability are calculated only for models that had 10 or less divergent transitions and converged. In addition the parameter recoverability metrics are only shown for models using the true link. \\
    \end{tablenotes}
  \label{tab:unit-descriptives}%
\end{threeparttable}%


==> tables/out-descriptives-positive.tex <==
\begin{threeparttable}
\caption{Descriptive Statistics of Lower-bounded Results}
  \centering
    \begin{tabular}{|l|l||r|r|r|r|r|r|r|r|r|}
\hline
  \rule{0pt}{3ex} Link & Likelihood & DT & $P(\text{Conv.})$ & $\mathrm{RESS}_{\rm bulk}$ & $\mathrm{RESS}_{\rm tail}$ &  $\mr{TESS_{total}^{bulk}}$ \\
    \hline
    Beta prime & Log & 0.012 (2.2) & 1 & 0.75 (0.18) & 0.66 (0.082) & 0.002 (0.018)\\ \hline Beta prime & Softplus & 0.004 (0.096) & 1 & 0.69 (0.16) & 0.64 (0.081) & 0.018 (0.57)\\ \hline Fréchet & Log & 0.73 (27) & 1 & 0.63 (0.16) & 0.59 (0.089) & 0.001 (0.065)\\ \hline Fréchet & Softplus & 298 (580) & 0.72 & 0.58 (0.15) & 0.56 (0.12) & 0.72 (6.2)\\ \hline Gamma & Log & 0.02 (5.3) & 1 & 0.85 (0.2) & 0.71 (0.074) & 0.46 (2.6)\\ \hline Gamma & Softplus & 0.023 (0.56) & 1 & 0.72 (0.17) & 0.65 (0.078) & 0 (0)\\ \hline Gompertz & Log & 99 (487) & 0.9 & 0.68 (0.16) & 0.63 (0.078) & 0.011 (0.47)\\ \hline Gompertz & Softplus & 7.3 (80) & 0.95 & 0.63 (0.17) & 0.61 (0.097) & 0.002 (0.001)\\ \hline Normal & Log & 2.4 (20) & 0.96 & 0.7 (0.18) & 0.63 (0.098) & 0.45 (3.3)\\ \hline Normal & Softplus & 0.68 (10) & 0.97 & 0.81 (0.21) & 0.67 (0.1) & 0.001 (0.072)\\ \hline trans. Normal & Log & 0 (0) & 1 & 0.85 (0.21) & 0.71 (0.074) & 0.3 (3.9)\\ \hline trans. Normal & Softplus & 0 (0) & 1 & 0.86 (0.21) & 0.71 (0.073) & 0.4 (2.8)\\ \hline Weibull & Log & 0.46 (22) & 1 & 0.8 (0.19) & 0.69 (0.075) & 0.001 (0)\\ \hline Weibull & Softplus & 0.34 (15) & 1 & 0.67 (0.16) & 0.62 (0.083) & 0.016 (0.59) \\
    \hline \hline
    \rule{0pt}{3ex} Link & Likelihood & PKs & $\mathrm{ELPD}_{\rm loo}$ & $\mathrm{bias}(\beta_{xy})$ & $\mathrm{SD}(\beta_{xy})$ & $\mathrm{RMSE}(\beta_{xy})$ \\
    \hline
    Beta prime & Log & 0.31 (0.57) & -190 (100) & 0.12 (0.13) & 0.07 (0.04) & 0.15 (0.12)\\ \hline Beta prime & Softplus & 0.33 (0.62) & -208 (84) & 0.2 (0.29) & 0.09 (0.06) & 0.24 (0.28)\\ \hline Fréchet & Log & 1.1 (1) & -186 (97) & 0.13 (0.14) & 0.08 (0.06) & 0.17 (0.14)\\ \hline Fréchet & Softplus & 0.95 (0.99) & -202 (107) & 0.15 (0.15) & 0.09 (0.06) & 0.19 (0.14)\\ \hline Gamma & Log & 0.19 (0.44) & -201 (66) & 0.15 (0.18) & 0.08 (0.08) & 0.18 (0.19)\\ \hline Gamma & Softplus & 0.52 (0.77) & -186 (95) & 0.13 (0.14) & 0.09 (0.07) & 0.18 (0.15)\\ \hline Gompertz & Log & 0.75 (0.89) & -188 (99) & 0.13 (0.14) & 0.08 (0.06) & 0.17 (0.14)\\ \hline Gompertz & Softplus & 0.97 (1.3) & -199 (106) & 0.6 (0.68) & 0.34 (0.26) & 0.75 (0.67)\\ \hline Normal & Log & 0.71 (0.92) & -222 (87) & 0.93 (1.2) & 0.43 (0.4) & 1.1 (1.2)\\ \hline Normal & Softplus & 0.36 (0.63) & -184 (109) & 0.5 (0.47) & 0.32 (0.18) & 0.65 (0.43)\\ \hline trans. Normal & Log & 0.21 (0.46) & -194 (126) & 0.57 (0.51) & 0.32 (0.18) & 0.71 (0.46)\\ \hline trans. Normal & Softplus & 0.25 (0.47) & -200 (86) & 0.56 (0.52) & 0.34 (0.18) & 0.71 (0.47)\\ \hline Weibull & Log & 0.4 (0.95) & -187 (113) & 0.53 (0.48) & 0.33 (0.17) & 0.68 (0.43)\\ \hline Weibull & Softplus & 0.87 (1.2) & -187 (112) & 0.5 (0.46) & 0.3 (0.15) & 0.64 (0.41) \\
    \hline
\end{tabular}%
     \begin{tablenotes}
      \tiny
      \item \textit{Note}: Most results are presented as mean(sd). $P(\text{Conv.})$ is calculated as a proportion of all models. $\mr{TESS_{total}^{bulk}}$ is also calculated using all models. Both the metrics for predictive performance and parameter recoverability are calculated only for models that had 10 or less divergent transitions and converged. In addition the parameter recoverability metrics are only shown for models using the true link. \\
    \end{tablenotes}
  \label{tab:positive-descriptives}%
\end{threeparttable}%


==> tables/out-descriptives-unit.tex <==
\begin{threeparttable}
\caption{Descriptive Statistics of Double-bounded Results}
  \centering
    \begin{tabular}{|l|l||r|r|r|r|r|r|r|r|r|}
\hline
  \rule{0pt}{3ex} Link & Likelihood & DT & $P(\text{Conv.})$ & $\mathrm{RESS}_{\rm bulk}$ & $\mathrm{RESS}_{\rm tail}$ &  $\mr{TESS_{total}^{bulk}}$ \\
    \hline
    Beta & Cauchit & 0 (0) & 1 & 0.84 (0.18) & 0.7 (0.073) & 0.001 (0.001)\\ \hline Beta & Cloglog & 0 (0) & 1 & 0.85 (0.17) & 0.72 (0.066) & 0.002 (0.002)\\ \hline Beta & Logit & 0 (0) & 1 & 0.87 (0.17) & 0.73 (0.065) & 0.14 (1.4)\\ \hline Kumaraswamy & Cauchit & 0 (0.026) & 1 & 0.73 (0.18) & 0.62 (0.11) & 0.001 (0.001)\\ \hline Kumaraswamy & Cloglog & 7.9 (105) & 0.97 & 0.81 (0.17) & 0.69 (0.066) & 0.001 (0.001)\\ \hline Kumaraswamy & Logit & 0 (0.004) & 1 & 0.78 (0.17) & 0.67 (0.068) & 0.001 (0.001)\\ \hline Normal & Cauchit & 0.012 (0.83) & 0.99 & 0.78 (0.2) & 0.63 (0.12) & 0.003 (0.17)\\ \hline Normal & Cloglog & 0.13 (2.1) & 0.95 & 0.83 (0.18) & 0.68 (0.088) & 0.62 (2.9)\\ \hline Normal & Logit & 0.018 (0.83) & 0.99 & 0.84 (0.19) & 0.69 (0.088) & 0.03 (0.38)\\ \hline Simplex & Cauchit & 0.83 (14) & 0.99 & 0.81 (0.2) & 0.69 (0.087) & 0.001 (0)\\ \hline Simplex & Cloglog & 22 (106) & 0.88 & 0.77 (0.21) & 0.67 (0.099) & 0.001 (0)\\ \hline Simplex & Logit & 0.46 (5.4) & 0.99 & 0.8 (0.2) & 0.7 (0.08) & 0.002 (0.001)\\ \hline trans. Normal & Cauchit & 0 (0) & 1 & 0.88 (0.18) & 0.72 (0.065) & 0.11 (1.1)\\ \hline trans. Normal & Cloglog & 0 (0) & 1 & 0.88 (0.18) & 0.72 (0.065) & 0.001 (0.001)\\ \hline trans. Normal & Logit & 0 (0) & 1 & 0.88 (0.18) & 0.72 (0.065) & 0.001 (0) \\
    \hline \hline
    \rule{0pt}{3ex} Link & Likelihood & PKs & $\mathrm{ELPD}_{\rm loo}$ & $\mathrm{bias}(\beta_{xy})$ & $\mathrm{SD}(\beta_{xy})$ & $\mathrm{RMSE}(\beta_{xy})$ \\
    \hline
    Beta & Cauchit & 0.024 (0.16) & 53 (28) & 0.21 (0.28) & 0.14 (0.06) & 0.28 (0.27)\\ \hline Beta & Cloglog & 0.021 (0.14) & 51 (29) & 0.34 (0.59) & 0.23 (0.21) & 0.44 (0.61)\\ \hline Beta & Logit & 0.015 (0.12) & 46 (36) & 0.27 (0.43) & 0.19 (0.15) & 0.35 (0.44)\\ \hline Kumaraswamy & Cauchit & 0.25 (0.52) & 48 (32) & 0.38 (0.71) & 0.23 (0.32) & 0.47 (0.77)\\ \hline Kumaraswamy & Cloglog & 0.23 (0.47) & 11 (81) & 0.67 (1.2) & 0.54 (0.78) & 0.93 (1.4)\\ \hline Kumaraswamy & Logit & 0.34 (0.56) & 53 (28) & 0.16 (0.18) & 0.1 (0.04) & 0.2 (0.17)\\ \hline Normal & Cauchit & 0.015 (0.13) & 52 (29) & 0.18 (0.22) & 0.14 (0.09) & 0.24 (0.22)\\ \hline Normal & Cloglog & 0.012 (0.11) & 46 (36) & 0.2 (0.28) & 0.13 (0.07) & 0.25 (0.27)\\ \hline Normal & Logit & 0.0054 (0.074) & 51 (28) & 0.19 (0.22) & 0.11 (0.05) & 0.23 (0.21)\\ \hline Simplex & Cauchit & 0.88 (1.4) & 51 (33) & 0.25 (0.35) & 0.18 (0.13) & 0.34 (0.35)\\ \hline Simplex & Cloglog & 0.96 (1.4) & 53 (28) & 0.21 (0.25) & 0.15 (0.06) & 0.27 (0.24)\\ \hline Simplex & Logit & 0.91 (1.3) & 52 (29) & 0.27 (0.38) & 0.19 (0.12) & 0.36 (0.37)\\ \hline trans. Normal & Cauchit & 0.73 (0.65) & 46 (36) & 0.26 (0.37) & 0.18 (0.1) & 0.34 (0.36)\\ \hline trans. Normal & Cloglog & 0.068 (0.26) & 49 (32) & 0.29 (0.38) & 0.17 (0.1) & 0.36 (0.37)\\ \hline trans. Normal & Logit & 0.052 (0.23) & 53 (28) & 0.33 (0.46) & 0.23 (0.16) & 0.43 (0.46) \\
    \hline
\end{tabular}%
     \begin{tablenotes}
      \tiny
      \item \textit{Note}: Most results are presented as mean(sd). $P(\text{Conv.})$ is calculated as a proportion of all models. $\mr{TESS_{total}^{bulk}}$ is also calculated using all models. Both the metrics for predictive performance and parameter recoverability are calculated only for models that had 10 or less divergent transitions and converged. In addition the parameter recoverability metrics are only shown for models using the true link. \\
    \end{tablenotes}
  \label{tab:unit-descriptives}%
\end{threeparttable}%

